How Many Data Samples is an Additional Instruction Worth?

Recently introduced instruction-paradigm empowers non-expert users to leverage NLP resources by defining a new task in natural language. Instruction-tuned models have significantly outperformed multitask learning models (without instruction); however they are far from state-of-the-art task-specific models. Conventional approaches to improve model performance via creating datasets with large number of task instances or architectural changes in the model may not be feasible for non-expert users. However, they can write alternate instructions to represent an instruction task. Is Instruction-augmentation helpful? We augment a subset of tasks in the expanded version of NATURAL INSTRUCTIONS with additional instructions and find that it significantly improves model performance (up to 35%), especially in the low-data regime. Our results indicate that an additional instruction can be equivalent to ~200 data samples on average across tasks.

==> table_single_task_results_averaged.tex <==
\begin{table}[t]
\large
\centering
\renewcommand{\arraystretch}{1.2}
{
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}c|llllllllll@{}}
\toprule

\multirow{2}{*}{\# of Instances} &  \multicolumn{2}{c}{SI} & \multicolumn{2}{c}{MVI}\\ 
\cmidrule(lr){2-5} 
~& Original & Ours & Original & Ours \\ 
\bottomrule
 1\% & 30.51 & 30.15 & 26.60 & 29.32 \\
 5\% & 29.79 & 68.83 & 26.00 & 69.10 \\
 10\% & 29.92 & 70.12 & 26.43 & 69.94 \\
 50\% & 69.91 & 72.91 & 64.14 & 72.74 \\
 100\% & 72.80 & 74.51 & 69.07 & 74.51 \\
\bottomrule
\end{tabular}
}
}
\caption{Comparison of LM Rouge-L performance in single-task setting averaged over 3 tasks across single-instruction and multi-variant instruction learning. SI: Single-Instruction, MVI: Multi-Variant Instruction.}
\label{tab:table_single_task_averaged}
\end{table}

==> table_single_task_results_task010.tex <==
\begin{table}[t]
\large
\centering
\renewcommand{\arraystretch}{1.2}
{
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}c|llllllllll@{}}
\toprule

\multirow{2}{*}{\# of Instances} &  \multicolumn{2}{c}{SI} & \multicolumn{2}{c}{MVI}\\ 
\cmidrule(lr){2-5} 
~& Original & Ours & Original & Ours \\ 
\bottomrule
 1\% & 0.00 & 0.00 & 0.00 & 0.02 \\
 5\% & 0.00 & 36.75 & 0.06 & 37.07 \\
 10\% & 0.23 & 39.17 & 0.15 & 38.26 \\
 50\% & 37.00 & 43.02 & 25.40 & 42.54 \\
 100\% & 41.97 & 45.65 & 33.84 & 45.50 \\
\bottomrule
\end{tabular}
}
}
\caption{Comparison of LM Rouge-L performance in single-task (task010) setting across single-instruction and multi-variant instruction learning. SI: Single-Instruction, MVI: Multi-Variant Instruction.}
\label{tab:table_single_task_task010}
\end{table}

==> table_single_task_results_task012.tex <==
\begin{table}[t]
\large
\centering
\renewcommand{\arraystretch}{1.2}
{
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}c|llllllllll@{}}
\toprule

\multirow{2}{*}{\# of Instances} &  \multicolumn{2}{c}{SI} & \multicolumn{2}{c}{MVI}\\ 
\cmidrule(lr){2-5} 
~& Original & Ours & Original & Ours \\ 
\bottomrule
 1\% & 84.48 & 83.54 & 75.45 & 82.66 \\
 5\% & 84.73 & 90.68 & 74.52 & 90.68 \\
 10\% & 84.81 & 90.61 & 75.47 & 90.60 \\
 50\% & 90.29 & 90.49 & 85.65 & 90.48 \\
 100\% & 90.84 & 90.50 & 88.47 & 90.52 \\
\bottomrule
\end{tabular}
}
}
\caption{Comparison of LM Rouge-L performance in single-task (task012) setting across single-instruction and multi-variant instruction learning. SI: Single-Instruction, MVI: Multi-Variant Instruction.}
\label{tab:table_single_task_task012}
\end{table}

==> table_single_task_results_task018.tex <==
\begin{table}[t]
\large
\centering
\renewcommand{\arraystretch}{1.2}
{
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}c|llllllllll@{}}
\toprule

\multirow{2}{*}{\# of Instances} &  \multicolumn{2}{c}{SI} & \multicolumn{2}{c}{MVI}\\ 
\cmidrule(lr){2-5} 
~& Original & Ours & Original & Ours \\ 
\bottomrule
 1\% & 7.05 & 6.92 & 4.36 & 5.27 \\
 5\% & 4.65 & 79.07 & 3.42 & 79.55 \\
 10\% & 4.72 & 80.59 & 3.68 & 80.95 \\
 50\% & 82.43 & 85.23 & 81.36 & 85.20 \\
 100\% & 85.58 & 87.37 & 84.90 & 87.52 \\
\bottomrule
\end{tabular}
}
}
\caption{Comparison of LM Rouge-L performance in single-task (task018) setting across single-instruction and multi-variant instruction learning. SI: Single-Instruction, MVI: Multi-Variant Instruction.}
\label{tab:table_single_task_task018}
\end{table}
